6G Radio Requirements to Support Integrated Communication, Localization, and Sensing

6G will be characterized by extreme use cases, not only for communication, but also for localization, and sensing. The use cases can be directly mapped to requirements in terms of standard key performance indicators (KPIs), such as data rate, latency, or localization accuracy. The goal of this paper is to go one step further and map these standard KPIs to requirements on signals, on hardware architectures, and on deployments. Based on this, system solutions can be identified that can support several use cases simultaneously. Since there are several ways to meet the KPIs, there is no unique solution and preferable configurations will be discussed.

==> bib/IEEEabrv.tex <==


IEEE Journals


aerospace and military
@STRING{IEEE_J_ANNE       = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AES        = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE        = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_AS         = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE       = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL        = "{IEEE} Trans. Mil. Electron."}



autos, transportation and vehicles (non-aerospace)
@STRING{IEEE_J_ITS        = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_IV         = "{IEEE} Trans. Intell. Veh."}
@STRING{IEEE_J_TTE        = "{IEEE} Trans. Transport. Electrific."}
@STRING{IEEE_J_VC         = "{IEEE} Trans. Veh. Commun."}
@STRING{IEEE_J_VT         = "{IEEE} Trans. Veh. Technol."}



circuits, signals, systems, audio and controls
@STRING{IEEE_J_STSP       = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SPL        = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_SYST       = "{IEEE} Syst. J."}
@STRING{IEEE_J_ASSP       = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU         = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA       = "{IEEE} Trans. Audio Electroacoust."}
in 2014 ASL became ASLP
@STRING{IEEE_J_ASLP       = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
@STRING{IEEE_J_ASL        = "{IEEE} Audio, Speech, Language Process."}
@STRING{IEEE_J_AC         = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS        = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT      = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI       = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII      = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CASI_RP    = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII_EB   = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT         = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST        = "{IEEE} Trans. Control Syst. Technol."}
@STRING{IEEE_J_ETCAS      = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
@STRING{IEEE_J_SP         = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_SU         = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP        = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE         = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC       = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}



communications
@STRING{IEEE_J_COML       = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC       = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM        = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT       = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM       = "{IEEE} Trans. Wireless Commun."}
@STRING{IEEE_J_WCOML      = "{IEEE} Wireless Commun. Lett."}



components, packaging and manufacturing
@STRING{IEEE_J_ADVP       = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT       = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
in 2011 CAPT became CPMT
@STRING{IEEE_J_CPMT       = "{IEEE} Trans. Compon. Packag. Manuf. Technol."}
@STRING{IEEE_J_CPMTA      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
@STRING{IEEE_J_CPMTB      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
@STRING{IEEE_J_CPMTC      = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPTS      = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CAPT       = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CPART      = "{IEEE} Trans. Compon. Parts"}
@STRING{IEEE_J_EPM        = "{IEEE} Trans. Electron. Packag. Manuf."}
@STRING{IEEE_J_MFT        = "{IEEE} Trans. Manuf. Technol."}
@STRING{IEEE_J_PHP        = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP        = "{IEEE} Trans. Parts, Mater., Packag."}



CAD
@STRING{IEEE_J_TCAD       = "{IEEE} J. Technol. Comput. Aided Design"}
@STRING{IEEE_J_CAD        = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}



coding, data, information, knowledge
@STRING{IEEE_J_BD         = "{IEEE} Trans. Big Data"}
@STRING{IEEE_J_IFS        = "{IEEE} Trans. Inf. Forensics Security"}
@STRING{IEEE_J_IT         = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE        = "{IEEE} Trans. Knowl. Data Eng."}



computers, computation, networking and software
@STRING{IEEE_J_CAL        = "{IEEE} Comput. Archit. Lett."}
@STRING{IEEE_J_ES         = "{IEEE} Embedded Syst. Lett."}
@STRING{IEEE_J_IOT        = "{IEEE} Internet Things J."}
@STRING{IEEE_J_XCDC       = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
@STRING{IEEE_J_MMCT       = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
@STRING{IEEE_J_SUSC       = "{IEEE} Sustain. Comput."}
@STRING{IEEE_J_CC         = "{IEEE} Trans. on Cloud Comput."}
@STRING{IEEE_J_CSS        = "{IEEE} Trans. Comput. Social Syst."}
@STRING{IEEE_J_C          = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_CNS        = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_DSC        = "{IEEE} Trans. Depend. Sec. Comput."}
@STRING{IEEE_J_ECOMP      = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_ETC        = "{IEEE} Trans. Emerg. Topics Comput."}
@STRING{IEEE_J_EVC        = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ       = "{IEEE} Trans. Fuzzy Syst."}
@STRING{IEEE_J_MC         = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_MSCS       = "{IEEE} Trans. Multi-Scale Comput. Syst."}
@STRING{IEEE_J_NET        = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NSE        = "{IEEE} Trans. Netw. Sci. Eng."}
@STRING{IEEE_J_NSM        = "{IEEE} Trans. Netw. Service Manag."}
@STRING{IEEE_J_NN         = "{IEEE} Trans. Neural Netw."}
in 2012 NN became NNLS
@STRING{IEEE_J_NNLS       = "{IEEE} Trans. Neural Netw. Learn. Syst."}
@STRING{IEEE_J_PDS        = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SC         = "{IEEE} Trans. Serv. Comput."}
@STRING{IEEE_J_SIPN       = "{IEEE} Trans. Signal Inf. Process. Netw."}
@STRING{IEEE_J_SE         = "{IEEE} Trans. Softw. Eng."}



computer graphics, imaging, and multimedia
@STRING{IEEE_J_JDT        = "{IEEE/OSA} J. Display Technol."}
@STRING{IEEE_J_IP         = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM         = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG        = "{IEEE} Trans. Vis. Comput. Graphics"}



cybernetics, ergonomics, robots, man-machine, artificial intelligence and automation
@STRING{IEEE_J_JAS        = "{IEEE/CAA} J. Autom. Sinica"}
@STRING{IEEE_J_JRA        = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_AFFC       = "{IEEE} Trans. Affect. Comput."}
@STRING{IEEE_J_ASE        = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_AMD        = "{IEEE} Trans. Auton. Mental Develop."}
@STRING{IEEE_J_CCN        = "{IEEE} Trans. on Cogn. Commun. Netw."}
in 2015 AMD became CDS
@STRING{IEEE_J_CDS        = "{IEEE} Trans. Cogn. Develop. Syst."}
@STRING{IEEE_J_CIAIG      = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
in 2013 SMCB became CYB
@STRING{IEEE_J_CYB        = "{IEEE} Trans. Cybern."}
@STRING{IEEE_J_H          = "{IEEE} Trans. Haptics"}
@STRING{IEEE_J_HFE        = "{IEEE} Trans. Hum. Factors Electron."}
in 2013 SMCC became HMS
@STRING{IEEE_J_HMS        = "{IEEE} Trans. Human-Mach. Syst."}
@STRING{IEEE_J_MMS        = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI       = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
in 1989 JRA became RA
in August 2004, RA split into ASE and RO
@STRING{IEEE_J_RA         = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_RAL        = "{IEEE} Robot. Autom. Lett."}
@STRING{IEEE_J_RO         = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC        = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA       = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB       = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC       = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
in 2012 SMCA became SMCS
@STRING{IEEE_J_SMCS       = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
@STRING{IEEE_J_SSC        = "{IEEE} Trans. Syst. Sci. Cybern."}



earth, wind, fire and water
@STRING{IEEE_J_GRSL       = "{IEEE} Geosci. Remote Sens. Lett."}
@STRING{IEEE_J_GE         = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS        = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE         = "{IEEE} J. Ocean. Eng."}
@STRING{IEEE_J_STARS      = "{IEEE} J. Sel. Topics Appl. Earth Observ. Remote Sens."}



education, engineering, history, IEEE, professional
@STRING{IEEE_J_CJECE      = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC       = "Proc. {IEEE}"}
@STRING{IEEE_J_RITA       = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
@STRING{IEEE_J_EDU        = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM         = "{IEEE} Trans. Eng. Manag."}
@STRING{IEEE_J_EWS        = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_LT         = "{IEEE} Trans. Learn. Technol."}
@STRING{IEEE_J_PC         = "{IEEE} Trans. Prof. Commun."}



electromagnetics, antennas, EMI, magnetics and microwave
@STRING{IEEE_J_AWPL       = "{IEEE} Antennas Wireless Propag. Lett."}
@STRING{IEEE_J_MAGL       = "{IEEE} Magn. Lett."}
@STRING{IEEE_J_MGWL       = "{IEEE} Microw. Guided Wave Lett."}
@STRING{IEEE_J_MWCL       = "{IEEE} Microw. Wireless Compon. Lett."}
@STRING{IEEE_J_RFIC       = "{IEEE} {RFIC} J."}
@STRING{IEEE_J_RFID       = "{IEEE} {RFID} J."}
@STRING{IEEE_J_AP         = "{IEEE} Trans. Antennas Propag."}
@STRING{IEEE_J_EMC        = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG        = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT        = "{IEEE} Trans. Microw. Theory Techn."}
@STRING{IEEE_J_RFI        = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TTHZ       = "{IEEE} Trans. {THz} Sci. Technol."}
@STRING{IEEE_J_TJMJ       = "{IEEE} Transl. J. Magn. Jpn."}



energy, power and conversion
@STRING{IEEE_J_PHOT       = "{IEEE} J. Photovolt."}
@STRING{IEEE_J_PEL        = "{IEEE} Power Electron. Lett."}
@STRING{IEEE_J_PETS       = "{IEEE} Power Energy Technol. Syst. J."}
@STRING{IEEE_J_ESTPE      = "{IEEE} Trans. Emerg. Sel. Topics Power Electron."}
@STRING{IEEE_J_EC         = "{IEEE} Trans. Energy Convers."}
@STRING{IEEE_J_PWRAS      = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD       = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE       = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS       = "{IEEE} Trans. Power Syst."}
@STRING{IEEE_J_SG         = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE        = "{IEEE} Trans. Sustain. Energy"}



industrial, commercial and consumer
@STRING{IEEE_J_PSE        = "{IEEE} J. Product Safety Eng."}
@STRING{IEEE_J_APPIND     = "{IEEE} Trans. Appl. Ind."}
@STRING{IEEE_J_BC         = "{IEEE} Trans. Broadcast."}
@STRING{IEEE_J_BCTV       = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE         = "{IEEE} Trans. Consum. Electron."}
@STRING{IEEE_J_IE         = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI       = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA         = "{IEEE} Trans. Ind. Appl."}
@STRING{IEEE_J_IGA        = "{IEEE} Trans. Ind. Gen. Appl."}
@STRING{IEEE_J_IINF       = "{IEEE} Trans. Ind. Informat."}



instrumentation and measurement
@STRING{IEEE_J_IM         = "{IEEE} Trans. Instrum. Meas."}



insulation and materials
@STRING{IEEE_J_JEM        = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI        = "{IEEE} Trans. Dielectr. Electr. Insul."}
@STRING{IEEE_J_EI         = "{IEEE} Trans. Electr. Insul."}



mechanical
@STRING{IEEE_J_MEMS       = "J. Microelectromech. Syst."}
in 2014 MEMS became MEMSI
@STRING{IEEE_J_MEMSI      = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MECH       = "{IEEE/ASME} Trans. Mechatronics"}



medical and biological
@STRING{IEEE_J_BHI        = "{IEEE} J. Biomed. Health Inform."}
@STRING{IEEE_J_TEHM       = "{IEEE} J. Transl. Eng. Health Med."}
@STRING{IEEE_J_LS         = "{IEEE} Life Sci. Lett."}
@STRING{IEEE_J_RBME       = "{IEEE} Rev. Biomed. Eng."}
@STRING{IEEE_J_BCAS       = "{IEEE} Trans. Biomed. Circuits Syst."}
@STRING{IEEE_J_BMELC      = "{IEEE} Trans. Bio-Med. Electron."}
B-ME later dropped the hyphen and became the BME
@STRING{IEEE_J_BME        = "{IEEE} Trans. Biomed. Eng."}
@STRING{IEEE_J_B-ME       = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_CBB        = "{IEEE/ACM} Trans. Comput. Biol. Bioinformatics"}
@STRING{IEEE_J_ITBM       = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME         = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI         = "{IEEE} Trans. Med. Imag."}
@STRING{IEEE_J_MBSC       = "{IEEE} Trans. Mol. Biol. Multi-Scale Commun."}
@STRING{IEEE_J_NB         = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE       = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
@STRING{IEEE_J_RE         = "{IEEE} Trans. Rehabil. Eng."}



optics, lightwave and photonics
@STRING{IEEE_J_JLT        = "J. Lightw. Technol."}
@STRING{IEEE_J_OCN        = "{IEEE} J. Opt. Commun. Netw."}
@STRING{IEEE_J_PJ         = "{IEEE} Photon. J."}
@STRING{IEEE_J_PTL        = "{IEEE} Photon. Technol. Lett."}



physics, electrons, nanotechnology, nuclear and quantum electronics
@STRING{IEEE_J_EDL        = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_EDS        = "{IEEE} J. Electron Devices Soc."}
@STRING{IEEE_J_JQE        = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE      = "{IEEE} J. Sel. Topics Quantum Electron."}
@STRING{IEEE_J_ENANO      = "{IEEE} Nanotechnol. Express"}
@STRING{IEEE_J_ED         = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO       = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS         = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS         = "{IEEE} Trans. Plasma Sci."}



reliability
@STRING{IEEE_J_DMR        = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R          = "{IEEE} Trans. Rel."}



semiconductors, superconductors, electrochemical and solid state
@STRING{IEEE_J_ESSL       = "{IEEE/ECS} Electrochem. Solid-State Lett."}
@STRING{IEEE_J_JSSC       = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC        = "{IEEE} Trans. Appl. Supercond."}
@STRING{IEEE_J_SM         = "{IEEE} Trans. Semicond. Manuf."}



sensors
@STRING{IEEE_J_SENSOR     = "{IEEE} Sensors J."}



VLSI
@STRING{IEEE_J_VLSI       = "{IEEE} Trans. {VLSI} Syst."}





IEEE Magazines and Online Publications


@STRING{IEEE_O_ACC        = "{IEEE} Access"}
@STRING{IEEE_M_AES        = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST       = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP         = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP       = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CHINAC     = "China Commun."}
@STRING{IEEE_M_CD         = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS        = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM        = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC     = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_O_CSTO       = "{IEEE} Commun. Surveys Tuts."}
@STRING{IEEE_M_CIM        = "{IEEE} Comput. Intell. Mag."}
CSEM changed to CSE in 1999
@STRING{IEEE_M_CSE        = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM       = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C          = "Computer"}
@STRING{IEEE_M_CAP        = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA        = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC       = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS         = "{IEEE} Control Syst. Mag."}
in 2012 DTC became DT
@STRING{IEEE_M_DT         = "{IEEE} Des. Test"}
@STRING{IEEE_M_DTC        = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_O_DSO        = "{IEEE} Distrib. Syst. Online"}
@STRING{IEEE_M_EI         = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETF        = "{IEEE} Electrific. Mag."}
@STRING{IEEE_M_EMC        = "{IEEE} Electromagn. Compat."}
@STRING{IEEE_M_ETR        = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMR        = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EMB        = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EXP        = "{IEEE} Expert"}
@STRING{IEEE_M_GRS        = "{IEEE} Geosci. Remote Sens. Mag."}
@STRING{IEEE_M_IA         = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IE         = "{IEEE} Ind. Electron. Mag."}
@STRING{IEEE_M_IM         = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS         = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_ITS        = "{IEEE} Intell. Transp. Syst. Mag."}
@STRING{IEEE_M_IC         = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP        = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO      = "{IEEE} Micro"}
@STRING{IEEE_M_MW         = "{IEEE} Microw. Mag."}
@STRING{IEEE_M_MM         = "{IEEE} Multimedia"}
@STRING{IEEE_M_NANO       = "{IEEE} Nanotechnol. Mag."}
@STRING{IEEE_M_NET        = "{IEEE} Netw."}
IEEE's editorial manual lists "Pers. Commun.",
but "Personal Commun. Mag." seems to be what is used in the journals
@STRING{IEEE_M_PCOM       = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_PVC        = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_POT        = "{IEEE} Potentials"}
@STRING{IEEE_M_PEL        = "{IEEE} Power Electron. Mag."}
CAP and PER merged to form PE in 2003
@STRING{IEEE_M_PE         = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER        = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PULSE      = "{IEEE} Pulse"}
@STRING{IEEE_M_RA         = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP        = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP         = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S          = "{IEEE} Softw."}
@STRING{IEEE_M_SSC        = "{IEEE} Solid-State Circuits Mag."}
@STRING{IEEE_M_SPECT      = "{IEEE} Spectr."}
@STRING{IEEE_M_SMC        = "{IEEE} Syst., Man, Cybern. Mag."}
@STRING{IEEE_M_TS         = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_VT         = "{IEEE} Veh. Technol. Mag."}
@STRING{IEEE_M_WC         = "{IEEE} Wireless Commun."}
@STRING{IEEE_M_TODAY      = "Today's Engineer"}





--
EOF

